Circumventing the CAP Theorem with Open {\AE}thernet

The CAP theorem is routinely treated as a systems law: under network partition, a replicated service must sacrifice either consistency or availability. The theorem is correct within its standard asynchronous network model, but operational practice depends on where partition-like phenomena become observable and on how lower layers discard or preserve semantic information about message fate. This paper argues that Open {\AE}thernet (OAE) shifts the engineering regime in which CAP tradeoffs become application-visible by (i) replacing fire-and-forget link semantics with bounded-time bilateral reconciliation of endpoint state -- the property we call bisynchrony -- and (ii) avoiding Clos funnel points via an octavalent mesh in which each node can act as the root of a locally repaired spanning tree. The result is not the elimination of hard graph cuts, but a drastic reduction in the frequency and duration of application-visible "soft partitions" by detecting and healing dominant fabric faults within hundreds of nanoseconds, under the link-fault model and repair rule stated in the paper. We connect this view to Brewer's original CAP framing, the formalization by Gilbert and Lynch, the CAL theorem of Lee et al., which replaces binary partition tolerance with a quantitative measure of apparent latency, and Abadi's PACELC extension.

==> acronyms.tex <==
\DeclareAcronym{AIT}{short = AIT, long = Reversible Token}
\DeclareAcronym{A2A}{short = A2A, long = Any to Any Addressing}
%\DeclareAcronym{E2E}{short = E2E, long = End to End Addressing}
\DeclareAcronym{ATST}{short = ATST, long = At the Same Time}
\DeclareAcronym{BKL}{short = BKL, long = Bypass Kleinberg Links}
\DeclareAcronym{CEQ}{short = CQ/EQ, long = Conserved Quantities/Exchanged Quantities}
\DeclareAcronym{complex}{short = complex, long = The set of cells reachable by this cell on its tree}
\DeclareAcronym{CAL}{short = CAL, long = Computation Asset Layer}
\DeclareAcronym{CAS}{short = CAS, long = Compare and Swap}
\DeclareAcronym{CEL}{short = \texttt{cell}, long = {Cell - an autonomous encapsulated single failure domain, containing processors, memory, storage and network processing}}
\DeclareAcronym{CDC}{short = CDC, long = Conventional Datacenter}
\DeclareAcronym{CK}{short = ECK, long = Consensus Klique}
\DeclareAcronym{CF}{short = TF, long = Transaction Fabrix}
\DeclareAcronym{CC}{short = CC, long = \href{https://en.wikipedia.org/wiki/Cargo_cult}{Cargo Cult}}
\DeclareAcronym{CRDT}{short = CRDTs, long = conflict-free replicated data type}
\DeclareAcronym{CLZ}{short = cluzter, long = A cluster of 9 cells where the center cell is the only one connected by 1 hop to all others}
\DeclareAcronym{CPU}{short = CPU, long = Central Processing Unit}
\DeclareAcronym{CNW}{short = CNW, long = Conventional Networking Wisdom}
\DeclareAcronym{GPU}{short = GPU, long = Graphics Processing Unit}
\DeclareAcronym{TPU}{short = TPU, long = Tensor Processing Unit}
\DeclareAcronym{DAG}{short = DAG, long = Directed Acyclic Graph}
\DeclareAcronym{DAL}{short = DAL, long = Data Asset Layer}
\DeclareAcronym{DC}{short = DC, long = Datacenter}
\DeclareAcronym{DL}{short = DL, long = Deep Learning}
\DeclareAcronym{DTA}{short = DTA, long = Dynamic Tree Algorithm}
\DeclareAcronym{DNN}{short = DNN, long = Deep Neural Network}
\DeclareAcronym{DPDK}{short = DPDK, long = \href{http://dpdk.org}{Data Plane Development Kit}}
\DeclareAcronym{DREDDFUL}{short = DReDDful, long = {Drop, Reorder, Delay and Duplicate}}
\DeclareAcronym{DVR}{short = DVR, long = Direct Vector Routing}
\DeclareAcronym{DUID}{short = DUID, long = Disposable Unique IDentifier}
\DeclareAcronym{ECF}{short = ECCF, long = Computing Cellular Fabric}
\DeclareAcronym{ECCF}{short = CF, long = DAE Computing Cellular Fabric}
\DeclareAcronym{EC}{short = EC, long = DAE Computing}
\DeclareAcronym{ECK}{short = ECK, long = DAE Consensus Klique}
\DeclareAcronym{ECN}{short = ECN, long = Explicit Congestion Notification}
\DeclareAcronym{ECLP}{short = ECLP, long = DAE Computing Link Protocol}
\DeclareAcronym{ECMP}{short = ECMP, long = Equal Cost Multi Path}
\DeclareAcronym{ELC}{short = ELC, long = \href{http://erights.org/elib/concurrency/event-loop.html}{Event Loop Concurrency}}
\DeclareAcronym{AELP}{short = AELP, long = Atomic Ethernet Liveness Protocol}
\DeclareAcronym{AETP}{short = AETP, long = Atomic Ethernet Token Protocol}
\DeclareAcronym{ENTL}{short = ENTL, long = Ethernet Non-Time Liveness}
\DeclareAcronym{ENTT}{short = ENTT, long = Ethernet Non-Time Transaction}
\DeclareAcronym{ENTP}{short = ENTL and ENTT, long = The DAE Non-Time Protocols}
\DeclareAcronym{EOD}{short = EOD, long = Exactly Once Delivery}
\DeclareAcronym{EOT}{short = EOT, long = Exactly Once Transmission}
\DeclareAcronym{EOR}{short = EOR, long = Exactly Once Reception}
\DeclareAcronym{EPI}{short = Epicycles, long = \href{https://en.wikipedia.org/wiki/Deferent_and_epicycle}{Epicycles} - the DAE-centric theory of planetary movement -- a metaphor for the network-centric theory of conventional datacenters}
\DeclareAcronym{E2E}{short = E2E, long = End to End Principle}
\DeclareAcronym{ESI}{short = ESI, long = Element of Shared Information}
\DeclareAcronym{FAQ}{short = FAQ, long = Frequently Asked Questions}
\DeclareAcronym{FE}{short = FE, long = Forwarding Engine}
\DeclareAcronym{FEFI}{short = FEFI, long = \href{https://www.transition.com/transition-networks-point-system-online-help/far-end-fault/}{Far End Fault Indication}}
\DeclareAcronym{FUD}{short = FUD, long = Fear Uncertainty and Doubt}
\DeclareAcronym{FLP}{short = FLP, long = {Fischer, Lynch and Patterson}}
\DeclareAcronym{GEV}{short = GEV, long = God's-Eye-View}
\DeclareAcronym{GVM}{short = GVM, long = Graph Virtual Machine}
\DeclareAcronym{IB}{short = IB, long = InfiniBand}
\DeclareAcronym{IBN}{short = IBN, long = InfiniBand Network}
\DeclareAcronym{HAL}{short = HAL, long = Hardware Abstraction Layer}
\DeclareAcronym{HOT}{short = HOT, long = Highly Optimized Tolerance}
\DeclareAcronym{IODAAS}{short = IoDaaS, long = In-order delivery -- \emph{as a service}}
\DeclareAcronym{IOMMU}{short = IOMMU, long = IO Memory Management Unit}
\DeclareAcronym{IP}{short = IP, long = Internet Protocol}
\DeclareAcronym{KVS}{short = KVS, long = Key Value Store}
\DeclareAcronym{LHL}{short = LHL, long = Logical Huang Links}
\DeclareAcronym{LKL}{short = LKK, long = Logical Kleinberg Link}
\DeclareAcronym{LOV}{short = LOV, long = Local Observer View}
\DeclareAcronym{LNK}{short = \texttt{link}, long = \texttt{link}}
\DeclareAcronym{LW}{short = LW, long = Leafward}
\DeclareAcronym{LSTM}{short = LSTM, long = \href{http://people.idsia.ch/~juergen/rnn.html}{Long-Short-Term Memory}}
\DeclareAcronym{LPAR}{short = LPAR, long = \href{https://en.wikipedia.org/wiki/Logical_partition}{Logical Partitions}}
\DeclareAcronym{MAC}{short = MAC, long = Media Access Control}
\DeclareAcronym{MEA}{short = MEA, long = Memory Equivalent Atomicity}
\DeclareAcronym{ML}{short = ML, long = Machine Learning}
\DeclareAcronym{MPA}{short = MPA, long = Message Passing Atomicity}
\DeclareAcronym{MSC}{short = MSC, long = Mutual State Coupling}
\DeclareAcronym{MVP}{short = MVPrototype, long = Minimum Viable Prototype}
\DeclareAcronym{NAL}{short = NAL, long = Network Asset Layer}
\DeclareAcronym{N2N}{short = N2N, long = Neighbor to Neighbor Addressing}
\DeclareAcronym{NDS}{short = NDS, long = Network Defined Software}
\DeclareAcronym{NFV}{short = NFV, long = Network Functions Virtualization}
\DeclareAcronym{NIC}{short = NIC, long = Network Interface Controler}
\DeclareAcronym{OCP}{short = \href{http://www.opencompute.org}{OCP}, long = Open Compute Project}
\DeclareAcronym{OUP}{short = OUP, long = Optimal Usable Product}
\DeclareAcronym{OAE}{short = OAE, long = Open Atomic Ethernet}
\DeclareAcronym{PCI}{short = PCIe, long = Peripheral Component Interconnect}
\DeclareAcronym{PAM}{short = PAM, long = Pulse Amplitude Modulation}
\DeclareAcronym{PFC}{short = PFC, long = Priority Flow Control}
\DeclareAcronym{PHL}{short = PHL, long = Physical Huang Links}
\DeclareAcronym{PLAY}{short = PLAY, long = Programmable Layer for Application Yakking}
\DeclareAcronym{PVR}{short = PVR, long = Path Vector Routing}
\DeclareAcronym{PQE}{short = PQE, long = Priority Queue Engine}
\DeclareAcronym{PKL}{short = PKL, long = Physical Kleinberg Links}
\DeclareAcronym{PMD}{short = PMD, long = \href{http://dpdk.org/doc/guides/prog_guide/poll_mode_drv.html}{Poll Mode Driver}}
\DeclareAcronym{QC}{short = QC, long = Quantum Computing}
\DeclareAcronym{QIT}{short = QIT, long = Quantum Information Theory}
\DeclareAcronym{QKD}{short = QKD, long = Quantum Key Distribution}
\DeclareAcronym{QPU}{short = QPU, long = Quantum Processing Unit}
\DeclareAcronym{QSFP}{short = QSFP, long = Quad Small Form-factor Pluggable}
\DeclareAcronym{QVM}{short = QVM, long = \href{http://pyquil.readthedocs.io/en/latest/examples.html}{Quantum Virtual Machine}}
\DeclareAcronym{RNG}{short = RNG, long = Random Number Generator}
\DeclareAcronym{RDMA}{short = RDMA, long = Remote Direct Access Memory}
\DeclareAcronym{REST}{short = REST, long = REpresentational State Transfer}
\DeclareAcronym{RCA}{short = RCA, long = Reversible Communication Atomicity}
\DeclareAcronym{RSM}{short = RSM, long = Replicated State Machine}
\DeclareAcronym{RFD}{short = RFD, long = Reliable Failure Detectors}
\DeclareAcronym{RPC}{short = RPC, long = Remote Procedure Call}
\DeclareAcronym{ROCE}{short = RoCE, long = RDMA over Converged Ethernet}
\DeclareAcronym{RCM}{short = RCM, long = RoCEv2 Congestion Management}
\DeclareAcronym{RNN}{short = RNN, long = \href{https://en.wikipedia.org/wiki/Recurrent_neural_network}{Recurrent Neural Network}}
\DeclareAcronym{ROV}{short = ROV, long = Remote-Observer-View}
\DeclareAcronym{RW}{short = RW, long = Rootward}
\DeclareAcronym{RAFE}{short = RAFE, long = Reliable Address Free Ethernet}
\DeclareAcronym{SDN}{short = SDN, long = Software Defined Network}
\DeclareAcronym{SDWAN}{short = SD-WAN, long = Software Defined Wide Area Networking}
\DeclareAcronym{SIB}{short = SIB, long = smooth (continuous) background (of time)}
\DeclareAcronym{SFP}{short = SFP+, long = Small Form-factor Pluggable}
\DeclareAcronym{SMA}{short = SMA, long = Shared Memory Atomicity}
\DeclareAcronym{SOC}{short = SOC, long = Self Organized Criticality}
\DeclareAcronym{SONIC}{short = SONiC, long = Software for Open Networking in the Cloud}
\DeclareAcronym{SPOF}{short = SPoF, long = Single Point of Failure}
\DeclareAcronym{SRIOV}{short = \href{https://en.wikipedia.org/wiki/Single-root_input/output_virtualization}{SR-IOV}, long = single root input/output virtualization}
\DeclareAcronym{SRS}{short = SRS, long = {\emph{Simplicity}, \emph{Resilience} \& \emph{Security}}}
\DeclareAcronym{SSM}{short = SSM, long = Shared State Machine}
\DeclareAcronym{SVL}{short = SVL, long = Sub-Virtualization Layer}
\DeclareAcronym{SWN}{short = SWN, long = `Small-Worlds'' Network}
\DeclareAcronym{TAC}{short = TAC, long = Topology Aware Computing}
\DeclareAcronym{TBA}{short = TBA, long = Tree-Based Addressing}
\DeclareAcronym{TF}{short = TF, long = Transition Fabrix}
\DeclareAcronym{TCB}{short = TCB, long = Trusted Computing Base}
\DeclareAcronym{TVR}{short = TVR, long = Tree Vector Routing}
\DeclareAcronym{TCT}{short = Treecast, long = \texttt{treecast}}
\DeclareAcronym{TICK}{short = \texttt{TICK}, long = \texttt{TICK}}
\DeclareAcronym{TOCK}{short = \texttt{TOCK}, long = \texttt{TOCK}}
\DeclareAcronym{TECK}{short = \texttt{TECK}, long = \texttt{TECK}}
\DeclareAcronym{TACK}{short = \texttt{TACK}, long = \texttt{TACK}} % not an ACK, it's a Thank You
\DeclareAcronym{TOR}{short = ToR, long = Top of Rack}
\DeclareAcronym{TTP}{short = TTP, long = Tiled Tree Paxos}
\DeclareAcronym{TIKTYKTIK}{short = \texttt{TIK\hspace{1pt}TYK\hspace{1pt}TIK}, long = The I Know That You Know That I Know property}
\DeclareAcronym{Treez}{short = Treez, long = Undirected Acyclic Subsets of a Datacenter Graph}
\DeclareAcronym{TRAPH}{short = TRee-grAPH, long = {A single tree subset of a Datacenter Graph $T(V,E')=G(V,E'\subseteq E)$}}
\DeclareAcronym{UAG}{short = UAG, long = Undirected Acyclic Graph}
\DeclareAcronym{UDLD}{short = UDLD, long = Uni-Directional Link Detection \href{https://en.wikipedia.org/wiki/Unidirectional_Link_Detection/}{}}
\DeclareAcronym{VHL}{short = VHL, long = Virtual Huang Links}
\DeclareAcronym{VKL}{short = VKL, long = Virtual Kleinberg Links}
\DeclareAcronym{VLSI}{short = VLSI, long = Very Large Scale Integration}
\DeclareAcronym{URT}{short = URT, long = Uniform Random Traffic}
\DeclareAcronym{WORC}{short = WORC, long = Wire-Oriented-Resilient-Consistency}
\DeclareAcronym{1PC}{short = 2PC, long = One-Phase Commit -- Send/Ack}
\DeclareAcronym{2PC}{short = 2PC, long = Two-Phase Commit}
\DeclareAcronym{3PC}{short = 3PC, long = Three-Phase Commit}
\DeclareAcronym{4PC}{short = 4PC, long = Four-Phase Commit}


==> dae-handout-commands.tex <==
% --- dae_commands.tex ---

% --- FAQ/Answer macros ---
\newcommand{\question}[1]{%
  \stepcounter{qctr}%
  \vspace{5pt}
  \noindent
  \rule{0.5\columnwidth}{0.5pt}\\
  \noindent
  \phantomsection
  \textbf{[Q\decimal{qctr}]}~%
  \def\a##1\par{##1}{#1}%
  \addcontentsline{loq}{section}{Q\protect\numberline{\theqctr}{{#1}}}
}

\newcommand{\answer}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}]}
}

\newcommand{\statement}{%
  \vspace{5pt}
  \noindent
  \textbf{[S\decimal{qctr}] Statement: }
}

\newcommand{\insight}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}} Insight: ]
}

\newcommand{\sublistofquestions}{%
  \onlyinsubfile{\vspace{0pt} \large \listofquestions \normalsize \medskip}
}

% --- Subfiles helpers ---
\newcommand{\onlyinsubfile}[1]{#1}
\newcommand{\notinsubfile}[1]{}

% --- Insert Hyperlink (file) ---
\newcommand{\ihl}[2]{%
  \vspace{6pt} \noindent [\hyperlink{./Exhibits/#1.pdf.1}{#1}]{ #2}
}

% --- Insert Menu Item (file/comment) ---
\newcommand{\imi}[2]{%
  \vspace{10pt}
  \noindent
  \textbf{\href{run:FAQ-#1.pdf}{#1}}\\{#2}
}

% --- Strikeout Displaystyle ---
\newcommand{\displayst}[1]{\textrm{\st{$\displaystyle#1$}}}

% --- Custom Horizontal Rule ---
\newcommand{\srule}{%
  \vspace{2pt}
  \noindent\rule{\textwidth}{0.8pt}
}

% --- Leibniz Bridge Margin TOC (standardized) ---
% Usage: place \daemargintoc after \maketitle / \placebadges on the first page.
% Requires: etoc, hyperref, linkgreen colour defined,
%           Bitstream Charter via mathdesign (provides bold small caps).
% Sections: bold small caps, green, with number.
% Subsections: regular small caps, green, indented.
% Section short titles MUST be in Title Case for the small-caps effect.
\newcommand{\daemargintoc}{%
  \marginnote{%
    \hypersetup{linkcolor=linkgreen}%
    \small
    \setcounter{tocdepth}{2}%
    \etocsetstyle{section}{}{\par\vspace{1em}\noindent\leftskip=0em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textbf{\textsc{\etocname}}}%
      \hfill\etocpage\par}{}{}%
    \etocsetstyle{subsection}{}{\par\vspace{0.5em}\noindent\leftskip=1.5em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textsc{\etocname}}%
      \hfill\etocpage\par}{}{}%
    \etocsettocstyle{}{}%
    \tableofcontents
  }%
}

\NewDocumentCommand{\marginfig}{O{width=\linewidth} m o o o o}{%
  \begin{marginfigure}\IfValueT{#6}{[#6]}%
    \IfValueTF{#5}{#5}{\centering}%
    \includegraphics[#1]{#2}%
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{marginfigure}
}

\NewDocumentCommand{\fig}{O{width=\linewidth} m o o}{%
  \begin{figure}
    \centering
    \includegraphics[#1]{#2}% 
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{figure}
}


==> dae-handout-settings.tex <==
% Document class

% Core packages
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}
\usepackage{xparse}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{lipsum}
\usepackage{epigraph}
\usepackage{framed}
\usepackage{todonotes}
\usepackage[most]{tcolorbox}

% Specialized
\usepackage{tikz}
\IfFileExists{bytefield.sty}{\usepackage{bytefield}}{}
\usepackage{eso-pic}

% Graphics path
\graphicspath{{./FIGURES/}{./figures/}{../Figures.}{../../Figures}{./images/}{./graphics/}{./FIGURES}}

% Hyperref
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  linkcolor=black,
  citecolor=black,
  urlcolor=blue
}

% Font commands
\newcommand{\headerfont}{\fontfamily{phv}\selectfont}
\newcommand{\titlefont}{\headerfont\Huge\bfseries}
\newcommand{\authorfont}{\headerfont\large}
\newcommand{\datefont}{\headerfont\normalsize}

% Custom title page
\makeatletter
\renewcommand{\maketitle}{
  \newpage
  \thispagestyle{empty}
  \begin{fullwidth}
    \centering
    {\titlefont \@title \par}
    \vspace{1em}
    \ifx\@author\@empty\else
      {\authorfont \@author \par}
      \vspace{0.5em}
    \fi
    \ifx\@date\@empty\else
      {\datefont \@date \par}
    \fi
    \vspace{2em}
  \end{fullwidth}
}
\makeatother

% Custom abstract
\newenvironment{customabstract}{
  \begin{fullwidth}
  \begin{adjustwidth}{0.5in}{0.5in}
  \vspace{1em}
  \small
  \color{gray!30!black}
}{
  \vspace{1.5em}
  \end{adjustwidth}
  \end{fullwidth}
}



% Unicode fallback
\DeclareUnicodeCharacter{2E3B}{\textbar\textbar}

% Optional: comment out subfiles you're not using
%\includeonly{Protocol-Byte-Content}

